Ray tracing methods for wave propagation in moving anisotropic media : application to magnetized plasmas

The propagation of a wave in a medium is generally affected when the medium is moving with respect to the observer. Because plasma equilibria often involve plasma flows, for instance in astrophysics or in magnetic confinement nuclear fusion devices, understanding the effect of motion on plasma waves is important. Meanwhile, the presence of a background magnetic field in a plasma makes it anisotropic. To address this problem, we derive here ray tracing equations for the trajectory of rays propagating in a moving anisotropic medium. The proposed approach is to use an effective dispersion relation for the moving medium as seen from the laboratory, obtained by performing a Lorentz transformation of the dispersion relation known for the medium at rest. This formalism is illustrated by considering the standard ordinary and extraordinary modes in a magnetized plasma at rest. Although we work here at lowest order in the geometrical optics approximation, this method is a first step towards higher order expansions, as required for instance to capture polarization effects.

==> CR-gen.tex <==
% We want to compile old articles (issues up to 2023) using the old template.
% Since the publication date is set in the .cfg file loaded after CR-gen.tex, we
% need to postpone the detection. It makes some of the code a bit heavier, but
% it is better than breaking everything.

\newif\ifcdr@oldtemplate
\ExplSyntaxOn
  \AtBeginDocument{
    \int_compare:nT {1 < \currentyear < 2024} {\cdr@oldtemplatetrue}
    \ifcdr@traduction \cdr@oldtemplatefalse \fi
    \ifcdr@oldtemplate
      \definecolor{cdr@accentcolor}{rgb}{0,0.6,.4} % AcademyGreen
    \fi
  }
\ExplSyntaxOff

\ifcdr@epreuves\RequirePackage[angle=60,scale=1.5,text={}]{draftwatermark}\fi
\ifcdr@epreuves\RequirePackage[pagewise,mathlines]{lineno}\fi
\ifcdr@traduction\RequirePackage[fitting,skins]{tcolorbox}\fi
\RequirePackage[absolute]{textpos}
\RequirePackage{cedram-graphics}
\RequirePackage[french,english,iso,cleanlook]{isodate} \origdate
\RequirePackage[shortlabels]{enumitem}

\def\currentjournaltitle{Comptes Rendus. \CDRcrasseries}
\def\currentjournalpublisher{Acad\'emie des sciences, Paris}
\def\journalURL{https://comptes-rendus.academie-sciences.fr/\cdr@journaldirectory/}%

\definecolor{cdr@accentcolor}{RGB}{125,103,255} % AcademyPurple

\let\cdr@rubricFR\@empty
\let\cdr@rubricEN\@empty
\let\cdr@presentedby\@empty
\let\cdr@resps\@empty
\let\cdr@specialtitle@english\@empty
\let\cdr@specialtitle@french\@empty

\def\cdr@printer@fr{}%{Imprim\'e en France par Sud Light Production / Clip (Centre Litt\'eraire d'impression Proven\c{c}al), Marseille, France}
\def\cdr@printer@en{}%{Printed in France by Sud Light Production / Clip (Centre Litt\'eraire d'impression Proven\c{c}al), Marseille, France}

\def\TopicFR#1{\gdef\cdr@topicFR{#1}}
\def\TopicEN#1{\gdef\cdr@topicEN{#1}}
\def\TopicEF#1#2{\gdef\cdr@topicEN{#1}\gdef\cdr@topicFR{#2}}
\def\RubricEF#1#2{
  \ClassError{cedram}{\noexpand\RubricEF is deprecated, use \string\CDRsetmeta{articletype}}{}
}

\ifcdr@LTXGrid
  \RequirePackage[papersize={192mm,262mm}, hmargin=16mm, vmargin={26.9mm,24.7mm}, foot=14mm, head=10pt, headsep=10mm]{geometry}
  \skip\footins=18ptplus12pt
  \abstractmargin6em
  \parskip0ptplus.1pt
  \floatsep 12pt plus 2pt minus 2pt
  \textfloatsep 20pt plus 2pt minus 4pt
  \intextsep 12pt plus 2pt minus 2pt
  \dblfloatsep 12pt plus 2pt minus 2pt
  \dbltextfloatsep 20pt plus 2pt minus 4pt
  \@fptop 0pt plus 1fil
  \@fpsep 8pt plus 2fil
  \@fpbot 0pt plus 1fil
  \@dblfptop 0pt plus 1fil
  \@dblfpsep 8pt plus 2fil
  \@dblfpbot 0pt plus 1fil
  \partopsep 2pt plus 1pt minus 1pt
  \def\clearlastpage@hook{\onecolumngrid\clearpage\eject}
  \def\@makefntext{\rule{0pt}{14pt}\@makefnmark}
\else
  \RequirePackage[papersize={192mm,262mm}, vmargin={26.9mm,24.7mm}, hmargin=26mm, foot=14mm, head=10pt, headsep=10mm]{geometry}
  \abstractmargin2em
\fi

\skip\@mpfootins=\skip\footins
\columnsep=18pt
\columnseprule=0pt
\abstractmarginL\abstractmargin
\abstractmarginR\abstractmargin
\marginparsep=10pt
\marginparpush=5pt
\marginparwidth=20mm
\pretolerance=600
\tolerance=2400 % INITEX sets this to 10000
\hbadness=2500
\vbadness=1000
\linepenalty=10
\hyphenpenalty=40
\exhyphenpenalty=50
\binoppenalty=700
\relpenalty=500
\clubpenalty=3000
\widowpenalty=4000
\displaywidowpenalty=6000
\brokenpenalty=3000
\predisplaypenalty=10000
\doublehyphendemerits=600
\finalhyphendemerits=4000
\adjdemerits=10000
\emergencystretch=1.5em
\uchyph=1
\hfuzz.5pt
\lineskip=0pt
\normalparindent=12pt
\parindent=\normalparindent
\captionindent=\normalparindent

\def\@mainsize{10}
\def\@ptsize{0}
\def\@typesizes{%
  \or{5}{6}\or{6}{7}\or{7}{8}\or{8}{10.1}\or{9}{11.2}%
  \or{10}{12.2}% normalsize
  \or{\@xipt}{13}\or{\@xiipt}{14}\or{\@xivpt}{17}%
  \or{\@xviipt}{20}\or{\@xxpt}{24}}%
\normalsize
\linespacing=\baselineskip

\let\@listI\@listi \@listi

\ifcdr@m@nuscript
  \ifluatex
    \RequirePackageIfExists{fourier-otf}{}
  \else
    \RequirePackageIfExists{fourier}{}
  \fi
  \let\sbseries=\bfseries
  \let\textsb=\textbf
\else
  \ifluatex
    \RequirePackage{amssymb}
    \RequirePackage[Scale=.98]{fourier-otf}
    \let\sbseries=\bfseries
    \let\textsb=\textbf
  \else
    \RequirePackage[expert]{fourier}
    \pdfmapfile{=fourier.map}
    \pdfmapfile{=fourier-utopia-expert.map}
  \fi
\fi

\def\@captionheadfont{\bfseries}
\def\cdr@up{}

\long\def\@makecaption#1#2{%
  \setbox\@tempboxa\vbox{\color@setgroup
    \advance\hsize-2\captionindent\noindent
    \@captionfont\@captionheadfont#1%
    \def\cdr@tmp@{\ignorespaces \ifHy@nesting \hyper@@anchor {\@currentHref }{}\else
      \Hy@raisedlink {\hyper@@anchor {\@currentHref }{\relax }}\fi}%
    \def\cdr@tmp@@{#2}%
%    \@xp\ifx\csname hyper@@anchor\endcsname\relax
    \ifx\cdr@tmp@@\cdr@tmp@\cdr@tmp@\else
    \def\cdr@tmp@{\ignorespaces}%
    \ifx\cdr@tmp@@\cdr@tmp@\else% \@xp\@ifnotempty\@xp{\@cdr#2\@nil}{
    \captionseparator\@captionfont\cdr@up\enspace#2
    \fi\fi
    \unskip\kern-2\captionindent\par
    \global\setbox\@ne\lastbox\color@endgroup}%
  \ifhbox\@ne % the normal case
    \setbox\@ne\hbox{\unhbox\@ne\unskip\unskip\unpenalty\unkern}%
  \fi
  % \ifdim\wd\@tempboxa=\z@ % this means caption will fit on one line
  %   \setbox\@ne\hbox to\columnwidth{\hss\kern-2\captionindent\box\@ne\hss}%
  % \else % tempboxa contained more than one line
    \setbox\@ne\vbox{\unvbox\@tempboxa\parskip\z@skip
        \noindent\unhbox\@ne\advance\hsize-2\captionindent\par}%
%  \fi
  \ifnum\@tempcnta<64 % if the float IS a figure...
    \addvspace\abovecaptionskip
    \hbox to\hsize{\kern\captionindent\box\@ne\hss}%
  \else % if the float IS NOT a figure...
    \hbox to\hsize{\kern\captionindent\box\@ne\hss}%
    \nobreak
    \vskip\belowcaptionskip
  \fi
\relax
}
%% unnumbered/unnamed captions
\def\silentcaption{%
   \ifx\@captype\@undefined
     \@latex@error{\noexpand\caption outside float}\@ehd
     \expandafter\@gobble
   \else
%     \refstepcounter\@captype
     \expandafter\@firstofone
   \fi
   {\@dblarg{\S@caption\@captype}}%
}
\long\def\S@caption#1[#2]#3{%
  \par
  \addcontentsline{\csname ext@#1\endcsname}{#1}%
    {\protect\numberline{\ }{\ignorespaces #2}}%
  \begingroup
    \@parboxrestore
    \if@minipage
      \@setminipage
    \fi
    \normalsize
    \S@makecaption{\csname fnum@#1\endcsname}{\ignorespaces #3}\par
  \endgroup}
\long\def\S@makecaption#1#2{%
  \setbox\@tempboxa\vbox{\color@setgroup
    \advance\hsize-2\captionindent\noindent
%    \@captionfont\@captionheadfont#1%
    \def\cdr@tmp@{\ignorespaces \ifHy@nesting \hyper@@anchor {\@currentHref }{}\else
      \Hy@raisedlink {\hyper@@anchor {\@currentHref }{\relax }}\fi}%
    \def\cdr@tmp@@{#2}%
%    \@xp\ifx\csname hyper@@anchor\endcsname\relax
    \ifx\cdr@tmp@@\cdr@tmp@\cdr@tmp@\else
    \def\cdr@tmp@{\ignorespaces}%
    \ifx\cdr@tmp@@\cdr@tmp@\else% \@xp\@ifnotempty\@xp{\@cdr#2\@nil}{
%    \captionseparator\@captionfont\cdr@up\enspace
#2
    \fi\fi
    \unskip\kern-2\captionindent\par
    \global\setbox\@ne\lastbox\color@endgroup}%
  \ifhbox\@ne % the normal case
    \setbox\@ne\hbox{\unhbox\@ne\unskip\unskip\unpenalty\unkern}%
  \fi
  % \ifdim\wd\@tempboxa=\z@ % this means caption will fit on one line
  %   \setbox\@ne\hbox to\columnwidth{\hss\kern-2\captionindent\box\@ne\hss}%
  % \else % tempboxa contained more than one line
    \setbox\@ne\vbox{\unvbox\@tempboxa\parskip\z@skip
        \noindent\unhbox\@ne\advance\hsize-2\captionindent\par}%
%  \fi
  \ifnum\@tempcnta<64 % if the float IS a figure...
    \addvspace\abovecaptionskip
    \hbox to\hsize{\kern\captionindent\box\@ne\hss}%
  \else % if the float IS NOT a figure...
    \hbox to\hsize{\kern\captionindent\box\@ne\hss}%
    \nobreak
    \vskip\belowcaptionskip
  \fi
\relax
}
%
%% Page layout
\pagenumbering{arabic}%
%% 1st page
\def\ps@firstpage{
  \ps@plain
  \def\@oddfoot{{\scriptsize
      \cdr@trans@get{eISSN}\hfill
      \hypersetup{linkcolor=cdr@accentcolor,urlcolor=cdr@accentcolor}
      \texttt{\url{\journalURL}}
  }}
  \let\@evenfoot\@oddfoot
  \let\@evenhead\@oddhead % in case an article starts on a left-hand page
}
%
%% Identificiation article 1st page
\def\@logofont{\footnotesize}
\def\cdr@subtitlesep{:}

\def\cdr@head{
  \ifcdr@oldtemplate
    \ifcdr@LTXGrid \vspace*{-2.3cm} \else \vspace*{-1.7cm} \fi
    \bgroup
    \@logofont \noindent
    {\Large\textit{Comptes Rendus\\ \CDRcrasseries}\\[2pt]}%
    \ifcdr@m@nuscript \textbf{Draft} \else
      \ifcdr@Attached
        \cdr@trans@get{supplementary}
      \else \ifcdr@efirst
        \ifx\@dateposted\@empty Not yet published%
        \else Published online: {\selectlanguage{english}\printdate{\@dateposted}}\fi
      \else
        \textbf{\currentyear}, Vol.~\currentvolume\displayissue{, }{, Special Issue }, p.\,\pageinfo
      \fi \fi
      \\\texttt{\printDOI}
    \fi
    \hfill\raisebox{-3mm}[0pt][0pt]{\includegraphics[height=16mm]{Logo_Academie_grisfonce.pdf}}%
    \ifcdr@Attached\else\\[18bp]%
      \centerline{\rule{.8\textwidth}{1.5bp}}%
    \fi
    \par \egroup
    \ifcdr@Attached \vspace{0.6cm} \fi
  \else
    \vspace*{-3cm}
    \bgroup
      \hspace{-1.5cm}\includegraphics[width=6cm]{CR_logo_h_black.pdf}
      \hfill
      \raisebox{1.2cm}{\begin{minipage}[b][][b]{9.5cm}
        {\hfill\Large\textit{\currentjournaltitle}\par}
        \hfill
        \ifcdr@m@nuscript
          \textbf{Draft}
        \else
          \ifcdr@Attached
            \cdr@trans@get{supplementary}
          \else
            \ifcdr@efirst
              \ifx\@dateposted\@empty\cdr@trans@get{unpublished}\else
                \if@francais En ligne depuis le \else Published online: \fi \printdate{\@dateposted}
              \fi
            \else
              \textbf{\currentyear}, Vol.~\currentvolume\displayissue{, }%
                {, \if@francais{\cdr@loc@numspecial@fr\ }\else{Special issue }\fi}, p.\,\pageinfo
            \fi
          \fi
          \par\hfill\texttt{\printDOI}
        \fi
      \end{minipage}}\hspace*{-.5cm}\par
      \vspace{-2ex}
      \centerline{\color{cdr@accentcolor}\rule{\paperwidth}{1mm}}
    \egroup
  \fi
}

\def\@maketitle@hook{
  \cdr@head
  \ifcdr@epreuves \linenumbers \fi
}
%% Standard pages
\def\ps@headings{%
    \ps@empty
    \def\@evenhead{%
        \rlap{\thepage}{}%\scshape
        \footnotesize\def\lastname####1{{####1}}%
        \hfil
        \def\thanks{\protect\thanks@warning}%
        \TopAuthors{}{}\hfil
    }%
    \def\@oddhead{%
        \let\\\relax
        \hfil
        \def\thanks{\protect\thanks@warning}%
        {\footnotesize\TopAuthors{}{}}\hfil
        \llap{\thepage}{}%
    }%
    \let\@mkboth\cdr@markboth
}
%
\ifnum \currentyear < \z@ \relax \def\currentyear{0000} \fi

\ifcdr@volume \else \pagestyle{headings} \fi
%
\setlength{\@titletopskip}{\topskip}
\setlength{\@titlebotskip}{0\p@}
%% title presentation

\let\overtitlebyhand\relax

\def\CDRtitleSep{~/ }

\cdr@ifeq{\cdr@mode}{bio}{
    \title{Guest editors}
    \alttitle{Rédacteurs invités}
    \let\TopAuthors=\relax
    \NewDocumentCommand {\guesteditor} {mm} {
        \begin{minipage}{.3\hsize}
            \centering
            \includegraphics[width=\hsize]{#2}\\
            \textbf{#1}
        \end{minipage}
    }
}{}

\cdr@var@load {..} {cdr@specialtitle@english} {}
\cdr@var@load {..} {cdr@specialtitle@french} {}
\ExplSyntaxOn
  \def\cdr@setarticletype{
    \prop_get:NnN \cdr_meta_prop {articletype} \l_tmpa_tl
    \if@francais
      \prop_get:NVN \cdr_articletypename_fr_prop \l_tmpa_tl \l_tmpb_tl \l_tmpb_tl
      \ifcdr@showtranslation \,/\, \prop_get:NVN \cdr_articletypename_en_prop \l_tmpa_tl \l_tmpb_tl \emph{\l_tmpb_tl} \fi
    \else
      \prop_get:NVN \cdr_articletypename_en_prop \l_tmpa_tl \l_tmpb_tl \l_tmpb_tl
      \ifcdr@showtranslation \,/\, \prop_get:NVN \cdr_articletypename_fr_prop \l_tmpa_tl \l_tmpb_tl \emph{\l_tmpb_tl} \fi
    \fi
  }
  \def\cdr@setarticletopic{
    \if@francais
      \cdr@topicFR \ifcdr@showtranslation\ifx\cdr@topicEN\@empty\else \,/\, \emph{\cdr@topicEN} \fi\fi
    \else
      \cdr@topicEN \ifcdr@showtranslation\ifx\cdr@topicFR\@empty\else \,/\, \emph{\cdr@topicFR} \fi\fi
    \fi
  }
  \def\@settitle{
    \begin{flushleft}
      \ifcdr@HideArticleType \else \bgroup \Large \cdr@setarticletype \par \egroup \fi
      \bgroup \Large \cdr@setarticletopic \par \egroup

      \ifx\TITREspecial\@empty\else \bgroup % This is part of a thematic issue
        \vspace{3ex} \LARGE
        \ifx\overtitlebyhand\relax
          \if@francais
            \let\cdr@specialtitle@main\cdr@specialtitle@french
            \let\cdr@specialtitle@alt\cdr@specialtitle@english
          \else
            \let\cdr@specialtitle@main\cdr@specialtitle@english
            \let\cdr@specialtitle@alt\cdr@specialtitle@french
          \fi
          \ifx\cdr@specialtitle@main\@empty
            \MissingInfo{\cdr@trans@get{Special-missing}}
          \else
            \ifcdr@swaptitles\@title\else\cdr@specialtitle@main\fi
            \ifx\cdr@specialtitle@alt\@empty\else
              \ifcdr@showtranslation\CDRtitleSep{\itshape\ifcdr@swaptitles\@alttitle\else\cdr@specialtitle@alt\fi}\fi
            \fi
          \fi
        \else
          \overtitlebyhand
        \fi
      \par \egroup \fi

      \vspace{3ex}

      {\Huge\ifcdr@swaptitles\cdr@specialtitle@english\else
        \@title
        \ifx\@subtitle\@empty\else \if@francais\,\fi :~ \@subtitle\fi
      \fi\par}

      \ifcdr@showtranslation
        { \if@francais\selectlanguage{french}\else\selectlanguage{english}\fi
          \huge\itshape
          \ifx\@alttitle\@empty\else
              \vspace*{14pt}
              \ifcdr@swaptitles\cdr@specialtitle@french\else
                  \ifcdr@Attached
                    \if@francais Supplementary ~ material: \else Document ~ compl\'ementaire\,: \fi ~
                  \fi\@alttitle % TODO French spacing for alt title
                  \ifx\@altsubtitle\@empty\else\if@francais\else\,\fi :~ \@altsubtitle\fi
              \fi
              \par
          \fi}
      \fi

      \vspace*{16pt}
    \end{flushleft}
  }
\ExplSyntaxOff
%

\let\@ESM\@empty
\newcommand\ESM[1]{\def\@ESM{#1}}

\def\cdr@preabstracthook{\par\bigskip}
\def\cdr@interabstracthook{\par}%\smallskip}
\def\cdr@postabstracthook{%
    \@@par\smallskip
    \ifx\@empty\@keywords\else
        \@@par\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setkeywords}\smallskip
    \fi
    \ifcdr@showtranslation\ifx\@empty\@altkeywords\else
        \@@par\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setaltkeywords}\smallskip
    \fi\fi
    \ifx\@empty\@subjclass\else
        \@@par\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setsubjclass}\smallskip
    \fi
    \ifx\@empty\thankses\else
        \@@par\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setthanks}\smallskip
    \fi
    \CDRifmeta {note}
    {\@@par\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setnote}\smallskip}
    {}
    \ifx\@empty\@ESM\else
        \@@par\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setESM}\smallskip
    \fi
    \@setpostabstractnotes
    \@@par{\abstractfont\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setdate}\par}
    \bigskip\bigskip
}
%
\def\abstractheadfont{\bfseries}
\def\@setabstracthead{{\abstractheadfont\abstractname\unskip.\kern.25em\ignorespaces}}
\def\@setaltabstracthead{{\abstractheadfont\altabstractname\unskip.\kern.25em\ignorespaces}%
}
%
%% authors
\def\@firstauthor#1\and#2\stop{#1}
\def\shortrunauthors{\gdef\@maketitle@shortauthors@hook{\def\topauthors{\@xp\@firstauthor\authors\stop\ \etal}}}
\def\shortrunPDGauthors{\g@addto@macro\@maketitle@shortauthors@hook{\def\PDGauthors{\@xp\@firstauthor\authors\stop\ \etal}}}
 \if@francais
  \def\manuscriptname{Manuscrit}%
  \def\receivedname{re\c cu}%
  \def\revisedname{r\'evis\'e}%
  \def\acceptedname{accept\'e}%
  \def\@@and{et}%
 \else
  \def\manuscriptname{Manuscript}%
  \def\receivedname{received}%
  \def\revisedname{revised}%
  \def\acceptedname{accepted}%
  \def\@@and{and}%
 \fi
%
\AtBeginDocument{\ifx\@daterevised\@dateaccepted\global\cdr@revisedacceptedtrue\fi
\ifx\@datereceived\@dateaccepted\global\cdr@receivedacceptedtrue\fi}
%
%%%%% presentation auteurs
%\def\@@and{\&}
 \def\author@andify{%
   \nxandlist {\unskip ,\penalty-2 \space\cdr@count@hasaddr=\z@\ignorespaces}%
     {\unskip {} \cdr@count@hasaddr=\z@\@@and~}%
     {\unskip {} \penalty-2  \cdr@count@hasaddr=\z@\@@and~}%
 }
% \def\@maketitle@shortauthors@hook{\msia@shortauthor@andify\shortauthors\let\topauthors\shortauthors}
\newcount\cdr@thankcount
\cdr@thankcount\z@
\ifcdr@LTXGrid\else
\def\@alph#1{\ifcase#1\or a\or b\or c\or d\else\@ialph{#1}\fi}
\def\@ialph#1{\ifcase#1\or \or \or \or \or e\or f\or g\or h\or i\or j\or
 k\or l\or m\or n\or o\or p\or q\or r\or s\or t\or u\or v\or w\or x\or
 y\or z\or aa\or bb\or cc\or dd\or ee\or ff\or gg\or hh\or ii\or jj\or
 kk\or ll\or mm\or nn\or oo\or pp\or qq\or rr\or ss\or tt\or uu\or
 vv\or ww\or xx\or yy\or zz\else\@ctrerr\fi}
\fi
\let\IsEqualContrib\relax
\let\IsCorresp\relax
\def\CDRfn#1#2{}
\newcount\CorrA\CorrA=\z@
\def\display@orcid#1{%
  \href{https://orcid.org/#1}{%
    \raisebox{.7ex}[0pt][0pt]{\includegraphics[height=1.1ex]{orcid-bw.png}}%
    }~}
\newcount\cdr@count@hasaddr\cdr@count@hasaddr=\z@%
\ExplSyntaxOn
  \def\dofn{
    \def\do##1##2{%
      \def\@thefnmark{\rule{0pt}{8pt}\llap{##1}}%
      \@footnotetext{##2}%
    }
    \def\dodo##1{\do##1}
    \seq_map_function:NN \cdr_fn_text_seq \dodo
  }
\ExplSyntaxOff
\def\@setauthors{%
  \begingroup
    \hsize=.9\linewidth \raggedright \large \sbseries
    \cdr@listauthors@cras\par
    \cdr@listnoauthors@cras{appendixwriter}{Appendix by }\par
    \dofn
  \endgroup
}%
\def\@setafterauthor{%
  \vglue3mm%
%  \hspace*{0pt}%
\begingroup\hsize=10cm\advance\hsize\abstractmarginL\raggedright
\noindent
%\hspace*{\abstractmarginL}\begin{minipage}[t]{10cm}
   \leftskip\abstractmarginL
  \normalfont\Small
  \@afterauthor\par
\endgroup
\vskip2pt plus 3pt minus 1pt
}
\def\@afterauthor{%
    \ifx\@empty\addresses\else
        \@setaddresses\par
        \ifcdr@GroupEmails
            \ifcdr@existcurraddr
                \@setcurraddr\par
            \fi
            \@setemails\par
        \fi
        \bigskip%
    \fi
    \ifx\postaddressinfo\relax\else\textbf{\postaddressinfo}\par\bigskip\fi
}
\newif\ifcdr@existcurraddr\cdr@existcurraddrfalse
\def\@setaddresses{\begingroup
  \cdr@thankcount\z@
  \url@samestyle
  \def\affiliationonly##1{##1}%
  \def\snailmailonly##1{\relax}%
  \def\lastname##1{\relax}%
  \def\firstname##1{\relax}%
  \def\hasthanks##1{##1\@addpunct.\@par}%
  \def\hasaddress##1{\relax}%
  \def\doauthorinfo##1{\@@par\textit{##1}}%
  \def\noauthor##1##2{}%
  \def\author##1{\def\\{ \ignorespaces}\ignorespaces}%
  \def\address##1##2{\begingroup
    \@ifempty{##1}{% cas pas addressSameAs
      \ifnum\cdr@thankcount>\z@\par\vskip4pt\fi\global\advance\cdr@thankcount\@ne
      \textsuperscript{\textit{\@alph\cdr@thankcount}}\kern.2em{\ignorespaces##2\unskip}}{}\endgroup}%
  \def\curraddr##1##2{%% Showing emails authorwise? Let's assume this follows the same logic as emails grouping.
    \ifcdr@GroupEmails\global\cdr@existcurraddrtrue\else\begingroup
      \@ifnotempty{##2}{\@@par\curraddrname{}\textit{\thsp:} %
      {\ignorespaces##2\unskip}\endgroup}\fi}%
  \def\email##1##2{%
    \ifcdr@GroupEmails\else\begingroup
      \@ifnotempty{##2}{\@@par\emailaddrname{}\@ifnotempty{##1}{ (##1)}\textit{\thsp:} \href{mailto:##2}{##2}}%
    \endgroup\fi}%
  \def\urladdr##1##2{\begingroup
    \@ifnotempty{##2}{\@@par\urladdrname{}\textit{\thsp:} %
      \url{##2}}\endgroup}%
  \addresses \endgroup}
\def\@setemails{\begingroup
  \cdr@thankcount\z@
  \url@samestyle
  \def\affiliationonly##1{\relax}%
  \def\snailmailonly##1{\relax}%
  \def\lastname##1{\relax}%
  \def\firstname##1{\relax}%
  \def\hasthanks##1{\relax}
  \def\hasaddress##1{\relax}%
  \def\noauthor##1##2{}%
  \def\author##1{}%
  \def\address##1##2{\relax}%
  \def\curraddr##1##2{\relax}%
  \def\doauthorinfo##1{\relax}%
  \def\email##1##2{%
    \ifcdr@GroupEmails\begingroup
      \@ifnotempty{##2}{\ifnum\cdr@thankcount=\z@\else, \fi\href{mailto:##2}{##2}\@ifnotempty{##1}{ \mbox{(##1)}}}%
    \endgroup\fi
    \global\advance\cdr@thankcount\@ne}%
  \def\urladdr##1##2{\relax}%
  \sbox\@tempboxa{\addresses\xdef\CDRess{\ifnum\cdr@thankcount>\@ne\relax s\fi}}%
  \ifdim\wd\@tempboxa>1em\relax
    \vskip2pt\@@par\textit{\emailsaddrname{}\CDRess\thsp:}
    \cdr@thankcount\z@
    \addresses%
  \fi
  \endgroup}
\def\@setcurraddr{%\par
  \begingroup
   \cdr@thankcount\z@
   \url@samestyle
   \def\affiliationonly##1{\relax}%
   \def\snailmailonly##1{\relax}%
   \def\lastname##1{\relax}%
   \def\firstname##1{\relax}%
   \def\hasthanks##1{\relax}
   \def\hasaddress##1{\relax}%
   \def\author##1{}%\ifnum\cdr@thankcount=\z@\else, \fi}
   \def\address##1##2{\relax}%
   \def\doauthorinfo##1{\relax}%
   \def\curraddr##1##2{%% Showing current addresses?
     \ifcdr@GroupEmails
     \begingroup
     \@ifnotempty{##2}{\ifnum\cdr@thankcount=\z@\else, \fi##2\@ifnotempty{##1}{ \mbox{(##1)}}}\endgroup\fi
     \global\advance\cdr@thankcount\@ne}%
   \def\email##1##2{\relax}%
   \def\urladdr##1##2{\relax}%
   \sbox\@tempboxa{\addresses\xdef\CDREss{\ifnum\cdr@thankcount>\@ne\relax es\fi}}%
   \ifdim\wd\@tempboxa>1em\relax
   \vskip2pt\@@par\textit{\curraddrname{}\CDREss\thsp:}
   \cdr@thankcount\z@
   \addresses%\@addpunct.%
   \fi
   \endgroup
 }

\def\@adminfootnotes{}

\def\@setsubjclass{%
  \abstractfont
  {\abstractheadfont\subjclassname.}\kern.25em\ignorespaces
  \@subjclass\@addpunct{{\upshape.}}\par}
\setlist{font=\upshape}
\newif\ifcdr@revisedaccepted\cdr@revisedacceptedfalse
\newif\ifcdr@receivedaccepted\cdr@receivedacceptedfalse
\newif\ifcdr@french@issue@title \cdr@french@issue@titlefalse
\def\daterevisedaccepted#1{%
  \def\@daterevised{#1}%
  \def\@dateaccepted{#1}%
  \cdr@revisedacceptedtrue
}
\def\@setdate{%
  \ifx\@empty\@dateaccepted
    \cdr@ifeq{\cdr@mode}{bio}{}{\MissingInfo{\cdr@trans@get{draft}}}%
  \else
    \if@francais
      \itshape\selectlanguage{french}%
      \noindent Manuscrit re\c cu
      \ifcdr@receivedaccepted
        et accept\'e le \printdate\@datereceived
      \else
        le \printdate\@datereceived,
        \ifcdr@revisedaccepted
          r\'evis\'e et  accept\'e le \printdate\@dateaccepted
        \else
          \ifx\@empty\@daterevised
          \else
            r\'evis\'e le \printdate\@daterevised
            \ifx\@empty\@datererevised
            \else
              \ et le \printdate\@datererevised
            \fi,
          \fi
          accept\'e le \printdate\@dateaccepted
        \fi
      \fi.
    \else
      \itshape\selectlanguage{english}%
      \noindent Manuscript
      received
      \ifcdr@receivedaccepted
        and accepted \printdate\@datereceived
      \else
        \printdate\@datereceived,
        \ifcdr@revisedaccepted
          revised and  accepted  \printdate\@dateaccepted
        \else
          \ifx\@empty\@daterevised
          \else
            revised \printdate\@daterevised
            \ifx\@empty\@datererevised
            \else
              \ and \printdate\@datererevised
            \fi,
          \fi
          accepted  \printdate\@dateaccepted
        \fi
      \fi.
    \fi
  \fi
}
\ifcdr@Thematic
\fi
%
\def\dedicatoryfont{\normalfont\footnotesize\itshape}
\def\@setdedicatory{%
    \begingroup
      \def\signature##1{\nobreak\hskip 2em plus 1fil
        \penalty-5\hbox{}\nobreak\hfil\parfillskip=0pt
        \mbox{\upshape ##1}\par}
      \raggedleft
      \dedicatoryfont
      \@dedicatory\par
    \endgroup}
\def\@setkeywords{%
  \global\kwd@count=\z@%
  \abstractfont%\hskip-\normalparindent
  {\abstractheadfont\keywordsname.}\kern.25em\ignorespaces
  \@keywords\unskip\@addpunct{{\upshape.}}\par}
\def\@setaltkeywords{%
  \global\kwd@count=\z@%
  \abstractfont%\hskip-\normalparindent
  {\abstractheadfont\altkeywordsname.}\kern.25em\ignorespaces
  \@altkeywords\unskip\@addpunct{{\upshape.}}\par}
\newcount\cdr@numberofthanks\cdr@numberofthanks=\z@
\def\@setthanks{\abstractfont\def\thanks##1{\ifnum\cdr@numberofthanks=\z@\relax\else\@par
   \fi##1\@addpunct{{\upshape.}}\advance\cdr@numberofthanks1\relax}{\abstractheadfont\thanksname.}\kern.25em\ignorespaces\thankses\par}
\def\@setnote{%
  \abstractfont%\hskip-\normalparindent
  {\abstractheadfont\notename.}\kern.25em\ignorespaces
  \CDRgetmeta{note}\@addpunct{{\upshape.}}\par}
\ExplSyntaxOn
  \NewDocumentCommand {\@setpostabstractnotes} {} {
    \bgroup
      \def\do##1##2{{\@@par\noindent\abstractfont {\abstractheadfont##1.}\kern.25em\ignorespaces
        ##2\@addpunct{{\upshape.}}\@@par\smallskip}}
      \seq_map_inline:Nn \cdr_note_seq {##1}
    \egroup
  }
\ExplSyntaxOff
\def\@setESM{%
  \abstractfont%\hskip-\normalparindent
  {\abstractheadfont\ESMname.}\kern.25em\ignorespaces
  \@ESM\@addpunct{{\upshape.}}\par}
\def\@settranslators{\par
  \begingroup
  \translatedby\ \andify\@translators
  {\sl \ignorespaces\@translators} \@@par
  \endgroup}
\if@francais
\def\cdr@correspondingname{Correspondance}
\def\keywordsname{Mots-cl{\'e}s}
\def\altkeywordsname{Keywords}
\def\subjclassname{Classification math{\'e}matique par sujets (2010)}
\def\thanksname{Financement}
\def\emailsaddrname{Courriel}
\def\notename{Note}
\def\ESMname{Mat{\'e}riel {\'e}lectronique suppl{\'e}mentaire}
\else
\def\cdr@correspondingname{Correspondance}
\def\keywordsname{Keywords}
\def\altkeywordsname{Mots-cl{\'e}s}
\def\subjclassname{Mathematical subject classification (2010)}
\def\thanksname{Funding}
\def\emailsaddrname{E-mail}
\def\notename{Note}
\def\ESMname{Electronic supplementary material}
\fi
\@xp\let\csname subjclassname@2010\endcsname \subjclassname
%
\def\longthankssection{\subsubsection*{Acknowledgements}}
\long\def\longthanks#1{\longthankssection

  #1}%
%
%
\def\enddoc@text{}
%
%% Page de garde
\def\@makePagedeGarde{
  \ifcdr@epreuves
    \SetWatermarkText{\normalfont PROOFS}
    \setlength\linenumbersep{.2cm}
  \fi
  \ifcdr@pagedegarde
    \ifcdr@traduction
      \input{CR-pagedegarde-traduction}
    \else
      \input{CR-pagedegarde}
    \fi
    \newpage
    \pagecolor{white}\gdef\GPT@pageliteral{}
  \else\ifcdr@epreuves
    \input{CR-pagedemetas}
    \newpage
    \pagecolor{white}\gdef\GPT@pageliteral{}
  \fi\fi
}
%
\ifcdr@sommaire % TODO: perhaps this is useless now
\let\cdr@postabstracthook\@empty
\def\ps@firstpage{\count@=\currentyear
  \ps@plain
  \let\@oddfoot\@empty
  \let\@evenfoot\@oddfoot
  \def\@oddhead{\@serieslogo\hss}%
  \let\@evenhead\@oddhead % in case an article starts on a left-hand page
}
%
\let\ps@headings\ps@empty
\let\ps@plain\ps@empty
\def\article@logo{%
    \set@logo{%
        \hsize\textwidth
        {\Large\textit{Comptes Rendus\\\CDRcrasseries}\\[2pt]}%
        \ifx\@empty\currentvolume
            \textbf{Draft}
        \else
            \textbf{\currentyear},
            \currentvolume
            \ifx\currentissue\@empty\else, \no\currentissue
        \fi\fi\\
        \mbox{}%
        \hfill
        \raisebox{-3mm}[0pt][0pt]{\includegraphics[height=16mm]{Logo_Academie_grisfonce.pdf}}\\[18bp]
        \centerline{\rule{.8\textwidth}{1.5bp}}
    }%
}
%
\def\smfbyname{\vspace*{-17mm}}
\def\lastname#1{#1}
\def\junior#1{\unskip, #1}%
\renewcommand{\@pnumwidth}{4.5em}
\def\@adminfootnotes{}
\def\enddoc@text{}
%%
\fi
\ifcdr@volume
    \cdr@InlineCouvtrue
    \cdr@InlineSomtrue
    \def\cdr@somhook{\small}
    \AtBeginDocument{\hypersetup{linkcolor=cdr@accentcolor,urlcolor=cdr@accentcolor}}
    \def\@makefront{%
        \IncludeSom
        \cleardoublepage
        \ifcdr@SOM
            % The point is to define cdr@resps and so on (for thematic issues)
            % the .cdrsom file is input by CR-couverture.tex
            % TODO this is much too complicated
            \@makeSOM
            \begingroup\makeatletter
                \newcommand\SomLine[9]{%
                    \gdef\cdr@resps{##2}%
                    \gdef\cdr@specialtitle@french{##5}%
                    \gdef\cdr@specialtitle@english{##4}%
                }%
                \InputIfFileExists{\jobname.cdrsom}{%
                    \message{** Fichier  \jobname.cdrsom charge  **^^J}}{%
                    \message{** Pas de fichier \jobname.cdrsom  pour ce volume !**^^J}}%
            \makeatother\endgroup
        \fi
    }
    \def\enddoc@text{}
    \renewcommand{\part}[1]{
        \ifcdr@somfileopen\else
            \immediate\openout\cdr@somfile=\CDRidvol.som
            \cdr@somfileopentrue
        \fi
        \immediate\write\cdr@somfile{\string\somtopic{#1}}

        \cleardoublepage
        \mbox{}
        \vfill
        \begin{center}
          \Huge\bf #1\par
        \end{center}
        \vfill
        \cleardoublepage
        \addtocounter{page}{-2}
    }
    \newcommand{\somtopic}[1]{
        \par\bigskip
        \begin{center}\Large\textsc{#1}\end{center}
        \nobreak
    }
\else % grab special volume editors from parent TODO: use \cdr@var@load for this
  \newcommand\SomLine[9]{
    \gdef\cdr@resps{#2}
    \gdef\cdr@specialtitle@french{#5}
    \gdef\cdr@specialtitle@english{#4}
  }
  \InputIfFileExists{../\CDRidvol.cdrsom}{}{}
\fi

%AJOUTS CS
%\RequirePackage{amssymb,upref}

\NumberTheoremsIn{}
\setcounter{tocdepth}{3}

%% Thms
\ifcdr@ThmDefs\OneNumberAllTheorems\fi
\def\th@plain{%
  \thm@bodyfont{\normalfont\itshape}%
  \thm@headfont{\normalfont\bfseries}%
  \thm@notefont{\normalfont\bfseries}%
  \thm@headpunct{.\kern.2em\ignorespaces}%
  \let\thm@indent\noindent
  \def\thm@space@setup{%
    \thm@preskip=\smallskipamount
    \thm@postskip=\thm@preskip}%
  \itshape
}
\def\th@remark{%
  \thm@bodyfont{\normalfont}%
  \thm@headfont{\normalfont\bfseries}%
  \thm@notefont{\normalfont\bfseries}%
  \thm@headpunct{.\kern.2em}%
  \let\thm@indent\noindent
  \def\thm@space@setup{%
    \thm@preskip=\smallskipamount
    \thm@postskip=\thm@preskip}%
}
\let\th@definition\th@plain
%\def\cdr@proofindent{\z@}%{1.5\parindent}
\renewenvironment{proof}[1][\proofname]{\par
  \pushQED{\qed}%
  \normalfont \topsep6\p@\@plus6\p@\relax
  \trivlist
  \item[\hskip\cdr@proofindent
        {\providecommand\printref{\relax}%
\bfseries
    #1\@addpunct{\cdr@proofpunct}}]\ignorespaces
}{%
  \popQED\endtrivlist\@endpefalse
}
%% Sectionning
\def\@startsection#1#2#3#4#5#6{%
 \if@noskipsec \leavevmode \fi
 \par \@tempskipa #4\relax
 \@afterindenttrue
 \ifdim \@tempskipa <\z@ \@tempskipa -\@tempskipa \@afterindentfalse\fi
 \if@nobreak \everypar{}\else
     \addpenalty\@secpenalty\addvspace\@tempskipa\fi
 \@ifstar{\@dblarg{\@sect{#1}{\@m}{#3}{#4}{#5}{#6}}}%
         {\@dblarg{\@sect{#1}{#2}{#3}{#4}{#5}{#6}}}%
}
\def\@seccntformat#1{%
  \protect\textup{\protect\@secnumfont
    \csname the#1\endcsname
    \protect\@secnumpunct
  }%
}
\def\@sectionfamily{\normalfont}
\def\@sectionfont{\@sectionfamily\large\bfseries}
\let\contentsnamefont\@sectionfont
\def\@secnumfont{\selectfont}
%\def\@upn{\normalfont\selectfont}
\def\@subsectionfont{\@sectionfamily\large\itshape}
\def\@subsubsectionfont{\@sectionfamily\itshape}
\def\@paragraphfont{\normalfont\bfseries}


\def\section{\@startsection{section}{1}%
  \z@{-1.5\linespacing\@plus-.5\linespacing\@minus-.5\linespacing}{.8\linespacing\@plus.2\linespacing\@minus.3\linespacing}%
  {\@sectionfont}}
\def\subsection{\@startsection{subsection}{2}%
  \z@{-1.5\linespacing\@plus-.5\linespacing\@minus-.5\linespacing}{.8\linespacing\@plus.2\linespacing\@minus.3\linespacing}%
  {\normalfont\@subsectionfont}}
\def\subsubsection{\@startsection{subsubsection}{3}%
  \z@{.5\linespacing\@plus.5\linespacing}{.5\linespacing}%
  {\normalfont\@subsubsectionfont}}
\def\paragraph{\@startsection{paragraph}{4}%
  \z@{.5\linespacing\@plus.5\linespacing}{-\fontdimen2\font}%
  {\normalfont\@paragraphfont}}
%
\newcount\tochyphenpenalty
\tochyphenpenalty\@M
\def\@tocline#1#2#3#4#5#6#7{\relax
  \ifnum #1>\c@tocdepth % then omit
  \else
    \par \addpenalty\@secpenalty\addvspace{#2}%
    \begingroup \hyphenpenalty\tochyphenpenalty
    \@ifempty{#4}{%
      \@tempdima\csname r@tocindent\number#1\endcsname\relax
    }{%
      \@tempdima#4\relax
    }%
    \parindent\z@ \leftskip#3\relax
      \advance\leftskip\@tempdima\relax
    \advance\rightskip\@pnumwidth % plus1em
    \parfillskip-\@pnumwidth
    {#5{\leavevmode\hskip-\@tempdima #6}}%
    \nobreak
    \xleaders\hbox to1ex{\normalfont\hss.\hss}\hfil\nobreak
    \hbox to\@pnumwidth{\@tocpagenum{#7}}\par
    \nobreak
    \endgroup
  \fi}
%
\renewcommand{\tocpart}[3]{%
  \indentlabel{\@ifnotempty{#2}{\ignorespaces#1 #2.\kern1ex}}#3}
\let\tocsection\tocpart
\let\tocsubsection\tocsection
\let\tocsubsubsection\tocsection
\let\tocparagraph\tocsection
\def\l@part{\@tocline{-1}{12pt plus2pt}{0pt}{}{\bfseries\smf@boldmath}}
\def\l@section{\@tocline{1}{0pt}{0pc}{}{}}
\def\l@subsection{\@tocline{2}{0pt}{1pc}{}{}}
\def\l@subsubsection{\@tocline{3}{0pt}{2pc}{}{}}
\def\l@paragraph{\@tocline{5}{0pt}{3pc}{}{}}
\def\l@figure{\@tocline{0}{3pt plus2pt}{0pt}{}{}}
\let\l@table\l@figure
%
\def\@smfprotect{\let\smfcr\\\def\\{\protect\smfcr}}
\DeclareRobustCommand{\MakeUppercase}[1]{{%
    \@smfprotect\upchars@
    \protected@edef\reserved@a{#1}\uppercasenonmath\reserved@a\reserved@a}}
\protected@edef\MakeUppercase#1{\MakeUppercase{#1}}
%
% \def\@makefnmark{%
%   \leavevmode
%   \raise.9ex\hbox{\fontsize\sf@size\z@\normalfont(\@thefnmark)}%
% }%CS
%
%% Additional macros %%
\AtBeginDocument{%
    \csname url@samestyle\endcsname
}
\emergencystretch2em
\arraycolsep 1.5pt
%%
\def\etal{{\normalfont\itshape et al.}}

\def\sautpage{\vadjust{\pagebreak}}
\newcommand\PB{\pagebreak}
\newcommand\SP{\sautpage}
\newcommand\SPB{\sautpage\break}
\newcommand\PBI{\pagebreak\noindent}

\def\orcid@link#1{\href{https://orcid.org/#1}{\includegraphics[height=1.5ex]{orcid-bw.png}}}

\ExplSyntaxOn
\NewDocumentCommand {\displayissue} {mm} {
  \ifx\currentissue\@empty\else
  \exp_args:NV \str_if_in:nnF \currentissue {G}
    {\exp_args:NV \str_if_in:nnTF \currentissue {S} {#2} {#1} \currentissue}
  \fi
}

\NewDocumentCommand {\cdr@typeset@person} {O{author}mm} { % #2 is index, #3 is name
  \bgroup
    \cdr_db_select_index_where_index_eq:Nnnn \l_tmpa_seq {address} {#1} {#2}
    \seq_set_map:NNn \l_tmpb_seq \l_tmpa_seq {\emph{\symbol{\numexpr96+##1}}}
    \seq_clear:N \l_tmpa_seq
    \def\CDRdecoration##1{\unskip\seq_put_right:Nn \l_tmpa_seq {##1}}
    \def\CDRfn##1##2{\CDRdecoration{##1}\cdr_fn_add_maybe:nn{##1}{##2}}
    \def\CDRorcid##1{\CDRdecoration{\orcid@link{##1}}}
    \def\IsCorresp{%
      \global\advance\CorrA\@ne\relax
      \CDRfn{$*$}{%
        \def\CDRss{\ifnum\CorrA>\@ne\relax s\fi}
        \if@francais Auteur\CDRss{} ~ correspondant\CDRss
        \else Corresponding ~ author\CDRss\vspace{-0.65cm}
        \fi}
    }
    \def\IsEqualContrib{%
      \CDRfn{$\#$}{\if@francais Contributions ~ \'egales\else Contributed ~ equally\fi}
    }
    \def\dead{%
      \CDRfn{$\dagger$}{\if@francais D\'ec\'ed\'e\else Deceased\fi}
    }
    \def\thanks{\protect\thanks@warning}
    #3
    \seq_map_inline:Nn \l_tmpb_seq {\seq_put_right:Nn \l_tmpa_seq {##1}}
    \seq_if_empty:NF \l_tmpa_seq
      { \, \@textsuperscript{\footnotesize \seq_use:Nn \l_tmpa_seq {,\hspace{.1em}}} }
  \egroup
}

\NewDocumentCommand {\cdr@list@authors} {O{author}} {
  \cdr_db_map_list:nnnnn {#1} { \cdr@typeset@person [#1] {##1} {##2} }
    {~{\@@and}~} {,~} {~{\@@and}~}
}

\def\cdr@listauthors@cras{\cdr@list@authors}

\def\cdr@listnoauthors@cras#1#2{
  \seq_if_in:NnT \cdr_db_contrib_seq {#1} {#2 \cdr@list@authors [noauthor]}
}
\ExplSyntaxOff

\ifluatex
  \babelfont[*cyrillic]{rm}{FreeSerif}
  \babelfont[thai]{rm}{FreeSerif}
\fi

\ifcdr@biblatex
  \AtEndOfClass{
    \let\cdr@addbibresource\addbibresource
    \renewcommand{\addbibresource}[1]{
      \cdr@addbibresource{#1}
      \IfFileExists{#1}{}{}
    }
  }
\fi

%%%%%%%%% Localization

\def\cdr@loc@redacinv@fr{R\'edacteur\CDRrss\ en chef invit\'e\CDRrss}
\def\cdr@loc@numspecial@fr{Num\'ero sp\'ecial}
